Randomized Response with Gradual Release of Privacy Budget

An algorithm is developed to gradually relax the Differential Privacy (DP) guarantee of a randomized response. The output from each relaxation maintains the same probability distribution as a standard randomized response with the equivalent DP guarantee, ensuring identical utility as the standard approach. The entire relaxation process is proven to have the same DP guarantee as the most recent relaxed guarantee. The DP relaxation algorithm is adaptable to any Local Differential Privacy (LDP) mechanisms relying on randomized response. It has been seamlessly integrated into RAPPOR, an LDP crowdsourcing string-collecting tool, to optimize the utility of estimating the frequency of collected data. Additionally, it facilitates the relaxation of the DP guarantee for mean estimation based on randomized response. Finally, numerical experiments have been conducted to validate the utility and DP guarantee of the algorithm.

==> unused.tex <==
Now we will prove the converse part of the above theorem.

\begin{lemma}
    For a set of queries $M_{\le n}$, if any outputs $y_{\le n}$ from $M_{\le n}$ satisfy $L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$, and a new query $M_{n+1}$ is not privacy-loss compactible with any queries in $M_{\le n}$, then $L(y_{\le n + 1}) = \sum\limits_{i = 1}^{n+1} \epsilon_i$ for any outputs from $M_{\le n + 1}$.
    % \begin{equation}
    %     \frac{\max\limits_x \prod\limits_x Pr(y_i | x)}{\min\limits_x \prod\limits_x Pr(y_i | x)} = 1
    % \end{equation}
\end{lemma}

\noindent Proof: we will prove it by contradiction. Assume $\exists y_{\le n + 1}: L(y_{\le n + 1}) < \sum\limits_{i = 1}^{n+1} \epsilon_i$. Also assume that $\forall y_{\le n}: L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$.
\begin{multline}
    \frac{\max\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)}{\min\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)} < \sum\limits_{i = 1}^{n+1} \epsilon_i = \\ \frac{\max\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x)}{\min\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x)}  \frac{\max\limits_x Pr(y_{n+1} | x)}{\min\limits_x Pr(y_{n+1} | x)} .
    \label{eq:K>1_to_compactible_step_1}
\end{multline}

\noindent Either $\max\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x) < \max\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x) \allowbreak \max\limits_x Pr(y_{n+1} | x)$ or  $\min\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x) > \min\limits_x \prod\limits_{i=1}^{n} \allowbreak Pr(y_i | x) \min\limits_x Pr(y_{n+1} | x)$. We assume the former, while the proof will be similar even if assuming the latter. Define $x_1 \in \argmax_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)$. Also define $\mathbf{x_2} = \allowbreak \argmax_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)$, and $\mathbf{x_3} = \argmax_x Pr(y_{n+1} | x)$, where $\mathbf{x_2}$ and $\mathbf{x_3}$ represent the set of $x$. It is easy to see $\mathbf{x_2} \cap \mathbf{x_3} = \emptyset$. Otherwise, $x_1 \in \mathbf{x_2} \cap \mathbf{x_3}$ and the Eq \eqref{eq:K>1_to_compactible_step_1} will be violated. Given $\forall y_{\le n}: L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$, we have $\forall x \in \mathbf{x_2}$ is also $\argmax_x Pr(y_j | x)$ where $j \le n$.

Consider $\forall u \in \argmax_x Pr(y_j | x_2) Pr(y_{n+1} | x)$. If $u \in \mathbf{x_2}$, then we have $u \notin \mathbf{x_3}$, so $ \exists y_{n+1}: Pr(y_{n+1} | u) < \max_x Pr(y_{n+1} | x)$. Therefore, we have $\exists y_{n+1}$:
\begin{multline}
    \max\limits_x Pr(y_j | x) Pr(y_{n+1} | x) <  \\ \max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x).
    \label{eq:K>1_to_compactible_step_2}
\end{multline}

\noindent Consequently,
\begin{multline}
    \frac{\max\limits_x Pr(y_j | x) Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x_2) Pr(y_{n+1} | x)} <  \frac{\max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x) Pr(y_{n+1} | x)} \\ \le  \frac{\max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x) \min \limits_x Pr(y_{n+1} | x)} = e^{\epsilon_j + \epsilon_{n+1}}.
\end{multline}

\noindent Therefore, $M_j$ and $M_{n+1}$ are privacy-loss compactible, which is contradicted to the condition of the Lemma. 

If $u \notin \mathbf{x_2}$, then $u$ cannot be both $\argmax_x \prod_{i = 1, i \ne j}^n Pr(y_i | x)$ and $\argmax_x Pr(y_j | x)$. If $u \notin \argmax_x Pr(y_j | x)$, then Eq. \eqref{eq:K>1_to_compactible_step_2} still holds, so does the consequent contradiction. If $u \notin \argmax_x \prod_{i = 1, i \ne j}^n Pr(y_i | x)$, then
\begin{multline}
    \max\limits_x \prod_{i = 1}^{n+1} Pr(y_i | x) < \\ \max\limits_x \prod_{i = 1, i \ne j}^{n+1} Pr(y_i | x) \max\limits_x [Pr(y_j | x) Pr(y_{n+1} | x)] . 
\end{multline}


\section{Branch and Bound}

Now, we will present the first version of branch-and-bound method (the same procedure as X). Recall that the queries introduced in Section \ref{sec:query_to_dc} requires each dimension of $x \in \mathcal{X}^m$ to have lower and upper bounds, and, for convenience, we call such constraints as a box constraint, denoted as $B^x$. The size of a box constraint is defined to the multiplication of all its lengths (the difference between upper and lower bounds). This method first computes the lower bound of $\min_x \log P(x)$ subject to $B^x$ (denoted as $LB(B^x)$) by solving $f(x) - \sum_i H_i(x)$ using convex optimization. Consider a box constraint $B_i^x$ whose feasible space belongs to that of $B^x$, denoted as $B_i^x \subset B^x$. Based on the definition of a concave envelope, we have $f(x) - \sum_i H_i(x) \rightarrow f(x) - g(x)$ when $\text{size}(B_i^x) \rightarrow 0$. Therefore, the method can converge $LB(B^x)$ to $\min_x \log P(x)$ by continuously split $B^x$ into smaller boxes. To do it, a priority queue is maintained to store all the split boxes. A box with lowest $LB$ will be picked up and split in half against one dimension of the box (i.e. a dimension of $x$). Assume this dimension has a bound of $[l, h]$. Then, the two newly-split boxes will have $[l, \frac{l+h}{2}]$ and $[\frac{l+h}{2}, h]$ as their new bounds of this dimension, while the bounds of other dimensions are unchanged. At the same time, the method computes the upper bound of $\min_x P(x)$ subject to the newly-split box constraint, denoted as $UB(B_i^x)$ where $B_i^x$ is the box constraint. $UB(B_i^x)$ can be acquired by any local optimization of the Difference of Convex Programming (hereinafter referred as LDC algorithm). The LDC algorithms usually utilize Newton Method and/or Sequential Linear Programming to find the local minimum. We choose the DCCP programming \cite{shen2016dccp} as its LDC algorithm. Additionally, the method maintains a global upper bound of $\min_x \log P(x)$ (denoted as $UB_g$) as $\min_{B_i^x \subset B^x}   UB(B_i^x)$. When the $LB$ of a box constraint is above $UB_g$, the method will discard this box without further splitting it. This method continues to run until all the (non-discarded) box constraints have $LB$ close enough to $UB_g$, and outputs $\min LB$ as a good enough lower bound for $\min_x \log P(x)$.

In practice, the $LB$ and $UB_g$ may converge slowly, so this method will be upgraded as follows. Recall that each $f_i(x)$ and $g_i(x)$ can be represented as $F(h(x))$, and denote $y = h(x)$; this gives an heuristic that the change of $f_i(x)$ and $g_i(x)$ is more sensitive to $y$ than $x$. When designing the branch-and-bound method, we could branch (split) on the $y$ of individual queries than $x$. Denote $\mathbf{Y} = \{Y_1, Y_2, ..., Y_n\}$, where $Y_i$ is a variable representing the output of $h_i(x)$. Given $x$ is bounded, each $Y_i$ will have lower and upper bounds, which can be considered as a box constraint on $\mathbf{Y}$, denoted as $B_0^\mathbf{Y}$. The above method is thus upgraded to split $B_0^\mathbf{Y}$ instead. The detail is at Algorithm \ref{algo:BnB}.
